Improving Generative Imagination in Object-Centric World Models

The remarkable recent advances in object-centric generative world models raise a few questions. First, while many of the recent achievements are indispensable for making a general and versatile world model, it is quite unclear how these ingredients can be integrated into a unified framework. Second, despite using generative objectives, abilities for object detection and tracking are mainly investigated, leaving the crucial ability of temporal imagination largely under question. Third, a few key abilities for more faithful temporal imagination such as multimodal uncertainty and situation-awareness are missing. In this paper, we introduce Generative Structured World Models (G-SWM). The G-SWM achieves the versatile world modeling not only by unifying the key properties of previous models in a principled framework but also by achieving two crucial new abilities, multimodal uncertainty and situation-awareness. Our thorough investigation on the temporal generation ability in comparison to the previous models demonstrates that G-SWM achieves the versatility with the best or comparable performance for all experiment settings including a few complex settings that have not been tested before.

==> tables/summary.tex <==
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccc}
\toprule
 & SQAIR & SILOT & SCALOR & STOVE \\
\midrule
% Discovery           & ? & ? & ? & ? \\
% Occlusion           & ? & ? & ? & ? \\
% Interaction         & ? & ? & ? & ? \\
% Two Layers          & ? & ? & ? & ? \\
% Two Layers Dense    & ? & ? & ? & ? \\
Discovery       & o & o & o & x  \\ 
Interaction     & x & x & x & o  \\ 
Occlusion       & o & o & o & x     \\
Scalability     & x & o & o & x  \\
Context         & x & x & o & x  \\ \hline 
% SSM & X & X & X & o  \\ \hline
Uncertainty    & x & x & x & x  \\
Situated        & x & x & x & x  
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
